Minimal Variance Sampling with Provable Guarantees for Fast Training of Graph Neural Networks

Sampling methods (e.g., node-wise, layer-wise, or subgraph) has become an indispensable strategy to speed up training large-scale Graph Neural Networks (GNNs). However, existing sampling methods are mostly based on the graph structural information and ignore the dynamicity of optimization, which leads to high variance in estimating the stochastic gradients. The high variance issue can be very pronounced in extremely large graphs, where it results in slow convergence and poor generalization. In this paper, we theoretically analyze the variance of sampling methods and show that, due to the composite structure of empirical risk, the variance of any sampling method can be decomposed into \textit{embedding approximation variance} in the forward stage and \textit{stochastic gradient variance} in the backward stage that necessities mitigating both types of variance to obtain faster convergence rate. We propose a decoupled variance reduction strategy that employs (approximate) gradient information to adaptively sample nodes with minimal variance, and explicitly reduces the variance introduced by embedding approximation. We show theoretically and empirically that the proposed method, even with smaller mini-batch sizes, enjoys a faster convergence rate and entails a better generalization compared to the existing methods.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> sections/method_2.tex <==
\subsection{MVS-GCN+}

\begin{algorithm2e}[t]
    \DontPrintSemicolon
    \caption{\texttt{Minimal Variance Sampling GCN + (MVS-GCN+)}}
    \label{algorithm:sgcn+}
    \textbf{input:} 
    initial point $\boldsymbol{\theta} = \{\mathbf{W}^{(1)}, \mathbf{W}^{(2)}, \cdots, \mathbf{W}^{(L)}\}$, learning rate $\eta$, $\{\boldsymbol{x}_i, y_i\}_{i\in\mathcal{V}}$, graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ \\
    Set $\mathbf{H}^{(0)} = \mathbf{X}$, mini-batch size $b$\\
    Let $\boldsymbol{p}=(p_1,p_2,\cdots,p_{|\mathcal{V}|})$ where $p_i = b/n$ and $w_i=1$ for all $i\in\mathcal{V}$\\
    \For{$t = 1,\cdots,T$}{
        \texttt{/* Run mini-batch GCN*/} \\
        Sample a subset of nodes $\mathcal{V}_\mathcal{B} \subseteq \mathcal{V}_\mathcal{L}$ using probability $\boldsymbol{p}$\\
        Construct $\{\tilde{\mathbf{L}}^{(\ell)}, \mathbf{L}^{(\ell)}\}_{\ell=1}^L$ that only contains nodes needed for $\mathcal{V}_\mathcal{B}$ \\
        \For{$\ell=1,\cdots,L$}{
            $\mathbf{Z}^{(\ell)} = (\tilde{\mathbf{L}}^{(\ell)} \mathbf{H}^{(\ell-1)} + \mathbf{L}^{(\ell)}\bar{\mathbf{H}}^{(\ell-1)}) \mathbf{W}^{(\ell)},~\mathbf{H}^{(\ell)} = \sigma(\mathbf{Z}^{(\ell)})$ \\
            $\bar{\mathbf{Z}}^{(\ell)} \leftarrow \mathbf{Z}^{(\ell)}$
        }
        Calculate gradient $\mathbf{g}_i = \nabla \ell(\mathbf{Z}^{(L)}_i, y_i)$ for $i \in \mathcal{V}_\mathcal{B}$ \\
        Update weight
        $\boldsymbol{\theta} \leftarrow \boldsymbol{\theta} - \eta \frac{1}{|\mathcal{V}_\mathcal{B}|} \sum_{i\in\mathcal{V}_\mathcal{B}} \mathbf{g}_i/p_i$ \\
        Calculate the sample distribution $w_i \leftarrow w_i \cdot \exp{\left(\frac{\delta \|\mathbf{g}\|^2}{n^2 p_i^3}\right)}$ for $i\in\mathcal{V}_\mathcal{B}$ \\
        Update $\mathbf{p}$ by $p_i \leftarrow (1-\eta) \frac{b w_i}{\sum_{i=1}^n w_i} + \frac{b \eta}{n}$ for $i \in \mathcal{V}$\\
        % $\boldsymbol{p}_b = \texttt{CalculateProbs}(\mathbf{g}, b\times\gamma)$ where $\boldsymbol{p}_b = (p_1,p_2,\cdots,p_{|\mathcal{V}_\mathcal{B}|})$ \\
        % Update $\mathbf{p}$ using $\mathbf{p}_b$ for $i\in\mathcal{V}_\mathcal{B}$.
    }
    \textbf{output:} 
    $\boldsymbol{\theta}$
\end{algorithm2e} 
Calculating the full-gradient and obtain the exact importance sampling distribution according to the per-sample gradient is computation expensive.
Instead of calculating the full-gradient and estimate the importance sampling distribution once a while, we first construct mini-batch by sampling nodes uniform at random, then we update the importance sampling probability for each node in that mini-batch. 


Suppose at each iteration, we sample a mini-batch from non-uniform distribution $\boldsymbol{p}_t = [p_{1,t},\cdots, p_{n,t}]$, where the probability $p_{i,t}$ of sampling data point $i$ at time $t$ is proportional to the upper bound of per-sample gradient norm $\hat{G}_{i,t}$. 
Denote $\mathbb{G}_t(\boldsymbol{p}) = \frac{1}{n^2}\sum_{i=1}^n(\hat{G}_{i,t}^2/p_i)$ as the stochastic gradient variance obtained at step $t$ by importance sampling distribution $\boldsymbol{p}$.
Let optimal solution $\boldsymbol{p}_t^\star$ denote the invariant distribution that minimize 
\begin{equation*}
    \boldsymbol{p}_t^\star = \underset{\boldsymbol{p}}{\arg\min}~ \mathbb{G}_t(\boldsymbol{p})
\end{equation*}
Our goal is to find an approximation solution of $\boldsymbol{p}^\star$ such that $\sum_{t=1}^T \mathbb{G}_t(\boldsymbol{p}_t) \leq c \sum_{t=1}^T \mathbb{G}_t(\boldsymbol{p}_t^\star)$ for some constant $c>1$.

\begin{restatable}{lemma}{batchmabsample}\label{lemma:batch_mab_sample}
Let $\boldsymbol{p}_t^\star$ be the optimal solution and $\boldsymbol{p}_t$ be the approximate solution at step $t$. Suppose the mini-batch size is $b$, we have
\begin{equation*}
    \sum_{t=1}^T \mathbb{G}_t(\boldsymbol{p}_t) \leq 3 \sum_{t=1}^T \mathbb{G}_t(\boldsymbol{p}_t^\star) + 50\sqrt{T \left(\sum_{i=1}^n \hat{G}_i^2\right) \ln{n}},
\end{equation*}
where $T> $
\end{restatable}
\begin{proof}
Proof can be found in Appendix \ref{appendix:batch_mab_sample}.
\end{proof}

==> trash/method_old.tex <==

In this section, we first derive the optimal sample distribution for minimal variance sampling, then we show the key challenge generalizing it to sampling-based GNNs. To overcome the issue, we propose a decoupled variance reduction approach, minimal variance sampling GNN (\texttt{MVS-GNN}), which perform zeroth- and first-order variance reduction to reduce the \emph{embedding approximation variance} and \emph{layer gradient variance}, respectively.

\begin{algorithm2e}[t]
    \DontPrintSemicolon
    \caption{\texttt{Minimal Variance Sampling GNN (MVS-GNN)}}
    \label{algorithm:sgcn+}
    \textbf{input:} 
    initial point $\boldsymbol{\theta} = \{\mathbf{W}^{(1)}, \mathbf{W}^{(2)}, \cdots, \mathbf{W}^{(L)}\}$, learning rate $\eta$, $\{\boldsymbol{x}_i, y_i\}_{i\in\mathcal{V}}$, graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ \\
    Set $\mathbf{H}^{(0)} = \mathbf{X}$, mini-batch size $b$ \\
    
    \For{$t = 1,\cdots,T$}{
        \texttt{/* Run Large-batch GNN*/} \\
        Sample a subset if nodes $\mathcal{V}_\mathcal{L}$ uniform at random\\
        Construct $\{\tilde{\mathbf{L}}^{(\ell)}\}_{\ell=1}^L$ that only contains nodes needed for $\mathcal{V}_\mathcal{L}$ \\
        $\bar{\boldsymbol{\theta}} = \{\bar{\mathbf{W}}^{(1)}, \bar{\mathbf{W}}^{(2)}, \cdots, \bar{\mathbf{W}}^{(L)}\} \leftarrow \boldsymbol{\theta} = \{\mathbf{W}^{(1)}, \mathbf{W}^{(2)}, \cdots, \mathbf{W}^{(L)}\}$\\
        \For{$\ell=1,\cdots,L$}{
            $\mathbf{Z}^{(\ell)} = \tilde{\mathbf{L}}^{(\ell)} \mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)},~ \mathbf{H}^{(\ell)} = \sigma(\mathbf{Z}^{(\ell)}) $ \\
            $\bar{\mathbf{Z}}^{(\ell)} \leftarrow \mathbf{Z}^{(\ell)}$ 
        }
        Calculate gradient $\mathbf{g} = (\mathbf{g}_1,\mathbf{g}_2, \cdots, \mathbf{g}_{|\mathcal{L}|})$ where $\mathbf{g}_i = \nabla \ell(\mathbf{Z}^{(L)}_i, y_i)$ for $i \in \mathcal{V}_\mathcal{L}$ \\
        Calculate the sample distribution $\boldsymbol{p} = \texttt{CalculateProbs}(\mathbf{g}, b)$ where $\boldsymbol{p} = (p_1,p_2,\cdots,p_{|\mathcal{V}_\mathcal{L}|})$ \\
        
        \texttt{/* Run mini-batch GNN*/} \\
        \For{$k= 1,\cdots, K$}{
            Sample a subset of nodes $\mathcal{V}_\mathcal{B} \subseteq \mathcal{V}_\mathcal{L}$ using probability $\boldsymbol{p}$\\
            Construct $\{\tilde{\mathbf{L}}^{(\ell)}, \mathbf{L}^{(\ell)}\}_{\ell=1}^L$ that only contains nodes needed for $\mathcal{V}_\mathcal{B}$ \\
            \For{$\ell=1,\cdots,L$}{
                $\mathbf{Z}^{(\ell)} = (\tilde{\mathbf{L}}^{(\ell)}\mathbf{H}^{(\ell-1)} + \mathbf{L}^{(\ell)}\bar{\mathbf{H}}^{(\ell-1)}) \mathbf{W}^{(\ell)},~\mathbf{H}^{(\ell)} = \sigma(\mathbf{Z}^{(\ell)})$ \\
                $\bar{\mathbf{Z}}^{(\ell)} \leftarrow \mathbf{Z}^{(\ell)}$
            }
            Calculate gradient $\mathbf{g}_i = \nabla \ell(\mathbf{Z}^{(L)}_i, y_i)$ for $i \in \mathcal{V}_\mathcal{B}$ \\
            Update weight
            $\boldsymbol{\theta} \leftarrow \boldsymbol{\theta} - \eta \frac{1}{|\mathcal{V}_\mathcal{B}|} \sum_{i\in\mathcal{V}_\mathcal{B}} \mathbf{g}_i/p_i$ \\
        }
    }
    \textbf{output:} 
    $\boldsymbol{\theta}$
\end{algorithm2e} 

\subsection{Minimal variance sampling}
The idea of minimal variance sampling is to reduce the stochastic gradient variance by choosing objects with larger loss gradient with higher probability than with smaller ones. This leads to a variance reduction of mini-batch estimated gradient and has a positive effect on model performance. In this section, we formulate the minimal variance sampling as an optimization problem and derive the closed-form nearly optimal solution. 

Formally, we consider the loss function and full-gradient as 
\begin{equation*}
    \mathcal{L} = \sum_{i=1}^N \ell(f(\boldsymbol{x}_i;\boldsymbol{\theta}), y_i),~
    \nabla \mathcal{L} = \sum_{i=1}^N \nabla \ell(f(\boldsymbol{x}_i;\boldsymbol{\theta}), y_i)
\end{equation*}

Rather than using all samples for each steps, we sample a sequence of random variable $\{\xi_i\}_{i=1}^{N}$, where $\xi_i \sim \mathrm{Bernoulli}(p_i)$, and $\xi_i=1$ indicates that $i$-th example is sampled and should be used to calculate the stochastic gradient $\mathbf{g}$:
\begin{equation*}
    \mathbf{g} = \sum_{i=1}^N \frac{\xi_i}{p_i} \nabla \ell(f(\boldsymbol{x}_i;\boldsymbol{\theta}), y_i)
\end{equation*} 
Define $\mathrm{Var}(\mathbf{g}) = \cE[\|\mathbf{g} - \cE[\mathbf{g}]\|^2]$. Our goal is to find the best set of $\{p_i\}_{i=1}^N$ such that minimize $\mathrm{Var}(\mathbf{g})$.
In this way, we come to the following form of minimization problem
\begin{equation*}\label{equation:1}
\begin{aligned}
    \underset{p_i}{\min} & \sum_{i=1}^N \frac{1}{p_i}\|\nabla \ell(f(\boldsymbol{x}_i;\mathbf{w}),y_i)\|^2 \\
    & \text{subject to } \sum_{i=1}^N p_i = n,~p_i\in(0,1] \text{ for all } i
    \end{aligned}
\end{equation*}
where $n$ is the expected sampled size for training.

Although this distribution can minimize the variance of the stochastic gradient, it requires the calculation of $N$ derivatives at each step, which is clearly inefficient. 
As stated in \cite{zhao2015stochastic,katharopoulos2018not}, a practical solution is to relax the optimization problem as follows
\begin{equation*}\label{equation:1_relax}
\begin{aligned}
    \underset{p_i}{\min} & \sum_{i=1}^N \frac{\hat{G}_i^2}{p_i} \\
    & \text{subject to } \sum_{i=1}^N p_i = n,~p_i\in(0,1] \text{ for all } i
    \end{aligned}
\end{equation*}
where $\hat{G}_i \geq \|\nabla \ell(f(\boldsymbol{x}_i;\mathbf{w}),y_i)\|$ is the upper-bound of the per-sample gradient norm.
Details can be found in Appendix \ref{appendix:upper_bound_grad_norm}.
\todo{do we need to put this in appendix? \cite{katharopoulos2018not} derived for neural network, i changed it to GNN, but the main idea is the same.}

\begin{theorem}\label{theorem:1}
 There exist a value $\mu$ such that $p_i = \min\left( 1, \frac{\hat{G}_i}{\mu} \right)$ is the solution of Equation \ref{equation:1_relax}.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{theorem:1}]
The Lagrange function of Equation \ref{equation:1_relax} has form:
\begin{equation*}
    L(\alpha,\beta_i,\gamma_i) = \sum_{i=1}^N \frac{\hat{G}_i^2}{p_i} + \alpha\left(\sum_{i=1}^N p_i - n\right) - \sum_{i=1}^N \beta_i p_i - \sum_{i=1}^N \gamma_i(1-p_i) 
\end{equation*}

By the KKT condition we know
\begin{equation*}
\left\{
\begin{array}{lr}
\frac{\partial L}{\partial p_i} = -\frac{\hat{G}_i^2}{p_i^2} + \alpha - \beta_i - \gamma_i = 0 \text{ for all } i &\\ 
\beta_i p_i = 0 \text{ for all } i & \\
\gamma_i(1-p_i) = 0 \text{ for all } i &
\end{array}\right.
\end{equation*}

Analyzing these conditions, it is easy to conclude that optimal solution has the following properties: (a) Since every $p_i>0$, we have $\beta_i=0$ for all $i$; (b) If $\gamma_i>0$, then $p_i=1$ and $\hat{G}_i^2 > \alpha + \gamma_i > \alpha$; (c) If $\gamma_i=0$, then $p_i = \sqrt{\hat{G}_i^2/\alpha}$.

Putting all together, we know that there exsit a threshold $\sqrt{\alpha}$ that divides sample into two parts $\{\boldsymbol{x}_i :\hat{G}_i > \sqrt{\alpha}\}$ of size $\kappa(\alpha)$ with $p_i=1$ and $\{\boldsymbol{x}_i :\hat{G}_i < \sqrt{\alpha}\}$ of size $N-\kappa(\alpha)$ with $p_i = \sqrt{\hat{G}_i^2/\alpha}$. 

Therefore, it is sufficient to find $\alpha=\alpha^\star$ such that $\sum_{i=1}^N p_i = n$. Desired value of $\alpha^\star$ can be found as a solution of 
\begin{equation*}
    \sum_{i=1}^N p_i = \sum_{i=1}^{N-\kappa(\alpha)} \sqrt{\frac{g^2_i}{\alpha}} + \kappa(\alpha) = n
\end{equation*}

We conclude the proof by setting $\mu=\sqrt{\alpha^\star}$.
\end{proof}
By Theorem \ref{theorem:1}, we know that given per-sample gradient, we can calculate a Bernoulli importance sampling distribution $\boldsymbol{p}:=\{p_i\}_{i=1}^N$ that minimize the variance. 
In Lemma \ref{lemma:bf_solution}, we give a brute-force algorithm relies on the dependence between sampling ratio and threshold, i.e., the higher the threshold, the lower the fraction of sampled instances.

\begin{lemma}\label{lemma:bf_solution}
Suppose $\hat{G}_i$ is sorted such that $0<\hat{G}_i\leq \cdots \leq \hat{G}_N$. Let $\kappa$ be the largest integer for which $n+\kappa-N \leq \hat{G}_i/(\sum_{i=1}^\kappa \hat{G}_i)$, then $\mu = (n+\kappa-N) / (\sum_{i=1}^\kappa \hat{G}_i)$. Then we have
\begin{equation*}
    p_i = 
    \begin{cases}
    (n+\kappa-N)\frac{\hat{G}_i}{\sum_{j=1}^\kappa \hat{G}_j} & \text{ if } i\leq \kappa \\
    1 & \text{ if } i > \kappa \\ 
    \end{cases}
\end{equation*}
\end{lemma}
\begin{proof} [Proof of Lemma \ref{lemma:bf_solution}]
The correctness of Lemma \ref{lemma:bf_solution} can be shown by plugging the result back to Theorem \ref{theorem:1}.
\end{proof}

\begin{remark}
The exact stochastic gradient variance obtain by sampling using $\boldsymbol{p}_{is}$ is calculated as 
\begin{equation*}
    \frac{1}{N^2}\sum_{i=1}^N \max\left\{1,~\frac{\sum_{j=1}^N \hat{G}_j}{(n+\kappa-N)\hat{G}_i}\right\} \hat{G}^2_i,
\end{equation*}
which is a function with respect to $\kappa$ defined in Lemma~\ref{lemma:bf_solution}. Comparing it with the variance of uniform sampling is not straight forward. Fortunately, the know the above equation is maximized if $\kappa=N$. Therefore in the following analysis, we considering the worst case where $\kappa=N$, and let $\mathbb{G}(\boldsymbol{p}_{is})$ to be 
\begin{equation*}
    \mathbb{G}(\boldsymbol{p}_{is}) = \frac{1}{N^2} \sum_{i=1}^N \frac{n \hat{G}_i}{\sum_{j=1}^N \hat{G}_j} \hat{G}_i^2
\end{equation*}
However, keep in mind that the exact variance obtained by our algorithm is always not worser than $\mathbb{G}(\boldsymbol{p}_{is})$.
\end{remark}

A more efficient way to find the value $\mu$ is by using the quick select algorithm.
First, we randomly select a gradient as a candidate to be a threshold of $\mu$. Then, the data is partitioned in such a way that all the instances with smaller gradients and larger gradients are on the opposite sides of the candidate. The current sample size $s(\mu)$ is calculated as 
\begin{equation*}
    s(\mu) = \frac{1}{\mu}\sum_{k+1}^N \hat{G}_i + k,
\end{equation*}
where $k$ is the number of elements with gradient $\hat{G}_i<s(\mu)$. 
Then, the estimated sample rate of $\mu$ is used to determine the side to continue the search for the desired threshold.

\todo{these algorithm can be removed}
The detailed algorithm of calculating $\boldsymbol{p}$ is detailed in Algorithm \ref{algorithm:calculate_probs} and the detailed algorithm of calculating $\mu$ is in Algorithm \ref{algorithm:calculate_thresh}.

% \subsection{Variance decomposition: forward versus backward}
% \todo{this part is similar to background \textbf{optimization problem} part. we can remove it}

% In the section, we show the mean-square error of the stochastic gradient can be decomposed as a function of \emph{embedding approximation variance} during forward propagation and \emph{stochastic gradient variance} during backward propagation.

% The mean-square error of the stochastic gradient estimator $\tilde{\mathbf{g}}$ is defined as $\cE[\|\tilde{\mathbf{g}}-\nabla f(\boldsymbol{\theta})\|^2]$. Using bias-variance decomposition, we can decompose mean-square error as 
% \begin{equation*}
%     \cE[\|\tilde{\mathbf{g}} - \nabla f(\boldsymbol{\theta})\|^2] = \cE[\|\tilde{\mathbf{g}} - \mathbf{g}\|^2] + \cE[\|\mathbf{g} - \nabla f(\boldsymbol{\theta})\|^2],
% \end{equation*}
% where $\cE[\tilde{\mathbf{g}}] = \mathbf{g}$. Next, we show in Lemma \ref{lemma:grad_bias} that the bias term $\cE[\|\tilde{\mathbf{g}} - \mathbf{g}\|^2]$ is a function of \emph{embedding approximation variance} which depends on the sampling algorithm, and show in Lemma \ref{lemma:grad_vars} that the variance term $\cE[\|\mathbf{g} - \nabla f(\boldsymbol{\theta})\|^2]$ is a function of sampling probability $p_i$ and the upper-bound of per-sample gradient norm, which can be minimized by selecting node with probability proportion to the upper-bound of per-sample gradient norm, i.e., $p_i\propto \hat{G}_i$.

%##################################
%##################################
% \begin{lemma}\label{lemma:grad_bias}
% Denote $\mathbb{V}_\ell$ as the upper-bound embedding approximation variance $\cE[\|f^{(\ell)}\circ \cdots \circ f^{(1)} - f_{\omega_\ell}^{(\ell)}\circ \cdots \circ f_{\omega_1}^{(1)}\|^2]$. Then we have
% \begin{equation*}
%     \cE[\|\mathbf{g}-\tilde{\mathbf{g}}\|^2] \leq L\cdot\sum_{\ell=1}^L \left(\prod_{i=1}^\ell \rho^2_i \right)\left(\prod_{i=\ell+1}^L \rho^2_i \right) L^2_\ell \cdot \mathbb{V}_\ell
% \end{equation*}
% \end{lemma}
%##################################
%##################################
% \begin{lemma}\label{lemma:grad_vars}
% Suppose $\hat{G}_i$ is the upper-bound of the per-sample gradient norm.
% Let $p_i$ be the probability of node $i$ get sampled in the mini-batch, then we have
% \begin{equation*}
%     \cE[\|\mathbf{g} - \nabla f(\boldsymbol{\theta})\|^2] \leq \frac{1}{N^2}\sum_{i=1}^N \frac{\hat{G}^2_i}{p_i}
% \end{equation*}
% \end{lemma}

% Therefore, using the result from Lemma \ref{lemma:grad_bias} and Lemma \ref{lemma:grad_vars}, we know that the mean-square error of GNN is bounded by
% \begin{equation*}
%     \cE[\|\tilde{\mathbf{g}} - \nabla f(\boldsymbol{\theta})\|^2] \leq \underbrace{L\cdot\sum_{\ell=1}^L \left(\prod_{i=1}^\ell \rho^2_i \right)\left(\prod_{i=\ell+1}^L \rho^2_i \right) L^2_\ell \cdot \mathbb{V}_\ell}_{\cE[\|\tilde{\mathbf{g}} - \mathbf{g}\|^2]} + \underbrace{\sum_{i=1}^N \frac{\hat{G}^2_i}{N^2 p_i}}_{\cE[\|\mathbf{g} - \nabla f(\boldsymbol{\theta})\|^2]}
% \end{equation*}
% Existing stochastic GNN training methods only focus on developing a better sampling strategy to improve the bias $\cE[\|\tilde{\mathbf{g}} - \mathbf{g}\|^2]$ by reducing the $\mathbb{V}_\ell$. However, in this paper we show that it is also essentially important to find the sample probability $p_i$ to reduce the stochastic gradient variance $\cE[\|\mathbf{g} - \nabla f(\boldsymbol{\theta})\|^2]$.
\subsection{MVS-GNN}


Although minimal variance sampling leads to variance reduction of the mini-batch estimated gradient, applying minimal variance sampling is not straight forward on sampling-based GNNs. To see this, let us consider a GNN with one graph convolutional layer and followed by one fully connected layer, which is general enough to illustrate the main difficulties, but is also relatively simple so that we can clearly explain the main ideas and techniques required to handle these difficulties. 

% \begin{equation*}
%     \begin{aligned}
%     &\texttt{ReLU}(\texttt{GraphConvolution}(\texttt{nfeat},  \texttt{nhid})) \\
%     &\texttt{LossFunction}(\texttt{Linear}(\texttt{nhid}, \texttt{nclass}), \texttt{Target})
%     \end{aligned}
% \end{equation*}

For the ease of presentation, let us represent the fully connected layer as $f(\boldsymbol{x};\boldsymbol{\theta}_f)$ and the graph convolutional layer as $g(\boldsymbol{x};\boldsymbol{\theta}_g)$.
Specifically, consider the loss function as
\begin{equation*}
    \mathcal{L} = \sum_{i=1}^N \ell\left(f(\boldsymbol{h}_i; \boldsymbol{\theta}_f), y_i\right),~
    \boldsymbol{h}_i = \sum_{j=1}^N g(\boldsymbol{x}_j;\boldsymbol{\theta}_g)
\end{equation*}
it's full gradient w.r.t. $\boldsymbol{\theta}_f, \boldsymbol{\theta}_g$ is calculated as
\begin{equation*}
    \begin{aligned}
    \nabla_{\boldsymbol{\theta}_f} \mathcal{L} &= \sum_{i=1}^N \frac{\partial \ell}{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)} \frac{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)}{\partial \boldsymbol{\theta}_f}\\
    \nabla_{\boldsymbol{\theta}_g} \mathcal{L} &= \sum_{i=1}^N \frac{\partial \ell}{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)} \frac{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)}{\partial \boldsymbol{h}_i} \sum_{j=1}^N \frac{\partial g(\boldsymbol{x}_j;\boldsymbol{\theta}_g)}{\partial \boldsymbol{\theta}_g}
    \end{aligned}
\end{equation*}

Rather than using all samples for each steps, we sample a sequence of random variable $\{\xi_i^f, \xi_i^g\}_{i=1}^{N}$, where $\xi_i^\star \sim \mathrm{Bernoulli}(p_i^\star)$, and $\xi_i^\star=1$ indicates that $i$-th example is sampled and should be used to calculate the stochastic gradient $\tilde{\nabla}_{\boldsymbol{\theta}_f} \mathcal{L}, \tilde{\nabla}_{\boldsymbol{\theta}_g} \mathcal{L}$:
\begin{equation*}
    \begin{aligned}
    \tilde{\nabla}_{\boldsymbol{\theta}_f} \mathcal{L} &= \sum_{i=1}^N \frac{\xi_i^f}{p_i}\frac{\partial \ell}{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)} \frac{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)}{\partial \boldsymbol{\theta}_f}\\
    \tilde{\nabla}_{\boldsymbol{\theta}_g} \mathcal{L} &= \sum_{i=1}^N \frac{\xi_i^f}{p_i}\frac{\partial \ell}{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)} \frac{\partial f(\boldsymbol{h}_i;\boldsymbol{\theta}_f)}{\partial \boldsymbol{h}_i} \sum_{j=1}^N \frac{\xi_j^g}{q_j}\frac{\partial g(\boldsymbol{x}_j;\boldsymbol{\theta}_g)}{\partial \boldsymbol{\theta}_g}
    \end{aligned}
\end{equation*}

Unfortunately, the optimal importance sampling distribution $\{p_i\}_{i=1}^N$ that minimize $\tilde{\nabla}_{\boldsymbol{\theta}_f} \mathcal{L}$ is different from the distribution that minimize $\tilde{\nabla}_{\boldsymbol{\theta}_g} \mathcal{L}$, which results in finding an optimal set of probability $\{p_i\}_{i=1}^N$ intractable. However, if we only sample nodes in the mini-batch, but use all its neighbors to inference the embedding matrix, the problem reduced to an \emph{exact-inference GNN} with $q_i=1$ for all $i\in[N]$, which can be solve by Algorithm \ref{algorithm:calculate_probs}.
% Therefore, the observation motivate us to use \emph{exact-inference GNN} to calculate the gradients for minimal variance sampling, which can be solve by Algorithm \ref{algorithm:calculate_probs}.

\begin{theorem}\label{theorem:sgcn_general_theorem}
Suppose function $f(\boldsymbol{\theta}_t)$ has $L_f$-Lipschitz continuous gradient.
Suppose we have access to the exact gradient to calculate the minimal variance sampling probability $p_i = \|\nabla f_i(\boldsymbol{\theta})\|/ \sum_{i=1}^n  \|\nabla f_i(\boldsymbol{\theta})\|$. By applying minimal variance sampling with parameters $\eta = \min\{\frac{1}{L_f}, \sqrt{\frac{\cE[f(\boldsymbol{\theta}_{1})] - \cE[f(\boldsymbol{\theta}_{*})]}{\tilde{\Delta} L_f T}}\}$, where $\tilde{\Delta}=\tilde{\Delta}_{is}$ for minimal variance sampling and $\tilde{\Delta}=\tilde{\Delta}_{us}$ for uniform sampling,
\begin{equation*}
    \begin{aligned}
    \tilde{\Delta}_{is} &= \sum_{i=1}^n \frac{\|\nabla f_i(\boldsymbol{\theta})\|^2}{n} + L\cdot\sum_{\ell=1}^L \left(\prod_{i=1}^\ell \rho^2_i \right)\left(\prod_{i=\ell+1}^L \rho^2_i \right) L^2_\ell \cdot \mathbb{V}_\ell \\
    \tilde{\Delta}_{us} &= \left( \sum_{i=1}^n \frac{\|\nabla f_i(\boldsymbol{\theta})\|}{n} \right)^2 + L\cdot\sum_{\ell=1}^L \left(\prod_{i=1}^\ell \rho^2_i \right)\left(\prod_{i=\ell+1}^L \rho^2_i \right) L^2_\ell \cdot \mathbb{V}_\ell
    \end{aligned}
\end{equation*}
with $n$ is the number of nodes sampled in the mini-batch.


Then, the corresponding output $\tilde{\boldsymbol{\theta}}$ satisfy $\cE[\|\nabla f(\tilde{\boldsymbol{\theta}})\|^2] \leq \epsilon$ provided that the total number $T$ of iterations satisfies
\begin{equation*}
    T \geq \cO(\tilde{\Delta}/\epsilon^2)
\end{equation*}
\end{theorem}
\begin{proof}
Proof can be found in Appendix \ref{appendix:convergence_analysis}.
\end{proof}

\begin{remark}
The result in Theorem \ref{theorem:sgcn_general_theorem} motivates us to develop an importance sampling strategy to sample nodes in the mini-batch that can reduce the gradient approximation variance, and develop a node sampling strategy that can reduce the embedding approximation variance at the same time.
\end{remark}

==> trash/warmup_old.tex <==
\todo{move stochastic gradient variance analysis to method section}
Next, we analysis the variance of stochastic gradient. For uniform sampling, nodes are sampled from distribution $\boldsymbol{p}_{us} = [p_1,\cdots, p_N]$ with $p_i = n/N$. For minimal variance sampling (importance sampling), nodes are sampled from distribution $\boldsymbol{p}_{is} = [p_1,\cdots, p_N]$ with $p_i=n\cdot g_i/(\sum_{i=1}^N g_i)$.
Define $\mathbb{G}(\boldsymbol{p}_{us})$ and $\mathbb{G}(\boldsymbol{p}_{is})$ as the the effective stochastic gradient variance of uniform sampling and importance sampling, respectively, where
\begin{equation*}
        \mathbb{G}(\boldsymbol{p}_{us}) = \frac{1}{nN} \sum_{i=1}^N g_i^2,~
        \mathbb{G}(\boldsymbol{p}_{is}) = \frac{1}{nN^2} \left(\sum_{i=1}^N g_i\right)^2
\end{equation*}
Then, we show in Lemma \ref{lemma:decouple_vars} the difference between $\mathbb{G}(\boldsymbol{p}_{us})$ and $\mathbb{G}(\boldsymbol{p}_{is})$.

\begin{lemma}\label{lemma:decouple_vars}
The difference between uniform sampling variance $\mathbb{G}(\boldsymbol{p}_{us})$ and importance sampling variance $\mathbb{G}(\boldsymbol{p}_{is})$ is proportional to the squared $\ell_2$ distance of the importance sampling distribution $\boldsymbol{p}_{is}$ to the uniform sampling distribution $\boldsymbol{p}_{us}$
\begin{equation*}
    \mathbb{G}(\boldsymbol{p}_{us})-\mathbb{G}(\boldsymbol{p}_{is}) = \frac{(\sum_{i=1}^N g_i)^2}{n^3 N} \|\boldsymbol{p}_{is}-\boldsymbol{p}_{us}\|_2^2
\end{equation*}
\end{lemma}
\begin{proof} [Proof of Lemma \ref{lemma:decouple_vars}]
\begin{equation*}
    \begin{aligned}
        \mathbb{G}(\boldsymbol{p}_{us})-\mathbb{G}(\boldsymbol{p}_{is}) &= \frac{1}{n} \sum_{i=1}^N \frac{g_i^2}{N} - \frac{1}{n } \left(\sum_{i=1}^N \frac{g_i}{N}\right)^2 \\
        &= \frac{(\sum_{i=1}^N g_i)^2}{n N^3}\sum_{i=1}^N \left( N^2 \frac{g_i^2}{(\sum_{i=1}^N g_i)^2}-1\right) \\
        &= \frac{(\sum_{i=1}^N g_i)^2}{n^3 N}\sum_{i=1}^N \left( \frac{n^2g_i^2}{(\sum_{i=1}^N g_i)^2}-\frac{n^2}{N^2}\right) \\
        &= \frac{(\sum_{i=1}^N g_i)^2}{n^3 N}\sum_{i=1}^N \left( \frac{ng_i}{\sum_{i=1}^N g_i}-\frac{n}{N}\right)^2 \\
        &= \frac{(\sum_{i=1}^N g_i)^2}{n^3 N} \|\boldsymbol{p}_{is}-\boldsymbol{p}_{us}\|_2^2
    \end{aligned}
\end{equation*}
\end{proof}


From Lemma \ref{lemma:mse_vars}, we know there are two types of variance when using sampling based training method: (a) \emph{stochastic gradient variance}: first-order variance that introduced during backward propagation and (b) \emph{function approximation variance}: zeroth-order variance that introduced during forward propagation.
Existing methods~\cite{chen2017stochastic,zou2019layer,chen2018fastgcn,zeng2019graphsaint} focus on developing a good sampling strategy to reduces \emph{embedding approximation variance}. However, they suffer from a high \emph{stochastic gradient variance} which slows down the convergence speed. 
Therefore, we propose \texttt{MVS-GNN} that uses minimal variance sampling to reduce the \emph{stochastic gradient variance} and use history activation of nodes from the previous layer to reduce the \emph{function approximation variance}, respectively.

% \begin{lemma}\label{lemma:convergence_rate_general}
% Suppose function $f(\boldsymbol{\theta}_t)$ has $L_f$-Lipschitz continuous gradient. The mean-square error (MSE) of stochastic gradient $\cE[\|\tilde{\mathbf{g}}_t-\nabla f(\boldsymbol{\theta}_t)\|^2] \leq \Delta$ is bounded by a constant $\Delta>0$. Set step size $\eta = \min\{\frac{1}{L_f}, \sqrt{\frac{\cE[f(\boldsymbol{\theta}_{1})] - \cE[f(\boldsymbol{\theta}_{*})]}{\Delta L_f T}}\}$ and let $\Tilde{\boldsymbol{\theta}} = \min_t \cE[\|\nabla f(\boldsymbol{\theta}_t)\|]$, we have
% \begin{equation*}
%     \cE[\|\nabla f(\Tilde{\boldsymbol{\theta}}_t)\|^2] \leq \sqrt{\frac{16L_f \Delta \left(\cE[f(\boldsymbol{\theta}_{1})] - \cE[f(\boldsymbol{\theta}_{*})]\right)}{T}}
% \end{equation*}
% \end{lemma}

\begin{lemma}\label{lemma:mse_vars}
Denote $\mathbb{V}_\ell$ as the upper-bound of embedding approximation variance of $\ell$th layer and $\mathbb{G}$ as the upper-bound of the stochastic gradient variance. Then we can decompose the MSE of stochastic gradient as
\begin{equation*}
    \begin{aligned}
     \cE_t[\|\tilde{\mathbf{g}}_t - \nabla F(\boldsymbol{\theta}_t)\|^2] &= \cE_t[\|\tilde{\mathbf{g}}_t - \mathbf{g}_t\|^2] + \cE_t[\|\mathbf{g}_t - \nabla F(\boldsymbol{\theta}_t)\|^2] \\
     &\leq L\cdot\sum_{\ell=2}^L \left(\prod_{i=1}^{\ell-1} \rho^2_i \right)\left(\prod_{i=\ell+1}^L \rho^2_i \right) L^2_\ell \cdot \left[ \sum_{j=1}^\ell \left(\sprod_{k=j+1}^\ell 2\rho^2_k \alpha^2_k \right) \cdot 2\rho^2_j \mathbb{V}_j \right] + \mathbb{G}
     \end{aligned}
\end{equation*}
\end{lemma}

From Lemma \ref{lemma:mse_vars}, we know there are two types of variance when using sampling based training method: (a) \emph{stochastic gradient variance}: first-order variance that introduced during backward propagation and (b) \emph{function approximation variance}: zeroth-order variance that introduced during forward propagation.
Existing methods~\cite{chen2017stochastic,zou2019layer,chen2018fastgcn,zeng2019graphsaint} focus on developing a good sampling strategy to reduces \emph{embedding approximation variance}. However, they suffer from a high \emph{stochastic gradient variance} which slows down the convergence speed. 
Therefore, we propose \texttt{MVS-GNN} that uses minimal variance sampling to reduce the \emph{stochastic gradient variance} and use history activation of nodes from the previous layer to reduce the \emph{function approximation variance}, respectively.

\paragraph{Variance comparison}
We compare the \emph{embedding approximation variance} and \emph{stochastic gradient variance} of different algorithms in Table \ref{table:01_vars}, we defer the detailed calculation to Appendix \ref{appendix:variance_analysis} and Appendix \ref{appendix:gradient_variance_analysis} for \emph{embedding approximation variance} and \emph{stochastic gradient variance}, respectively. 

On the one hand,
we highlight the difference of embedding approximation variance with existing sampling based method. Compare with sampling based methods without Zeroth-order variance reduction (such as GraphSage, LADIES, and GraphSaint), our method enjoys a lower variance since $\Delta \beta_\ell^2 \ll \beta_\ell^2$. Compared with sampling based method with Zeroth-order variance reduction (such as VRGNN), our algorithm has a higher variance, however the computation complexity and sampling complexity is much lower. 

On the other hand,
we highlight in Lemma \ref{lemma:us_vs_is} the difference between $\mathbb{G}(\boldsymbol{p}_{us})$ and $\mathbb{G}(\boldsymbol{p}_{is})$ where
\begin{equation*}
    \mathbb{G}(\boldsymbol{p}_{us}) = \frac{1}{N^2} \sum_{i=1}^N \frac{N}{n}g_i^2,~\mathbb{G}(\boldsymbol{p}_{is}) = \frac{1}{N^2} \sum_{i=1}^N \frac{\sum_{j=1}^N g_j}{ng_i} g^2_i
\end{equation*}
We show that $\mathbb{G}(\boldsymbol{p}_{is})\leq\mathbb{G}(\boldsymbol{p}_{us})$, and $\mathbb{G}(\boldsymbol{p}_{is})=\mathbb{G}(\boldsymbol{p}_{is})$ if and only if the importance sampling distribution is the same as uniform sampling distribution.

\begin{restatable}{lemma}{usvsis}\label{lemma:us_vs_is}
% Let $\boldsymbol{p}_{us} = [p_1,\cdots,p_N]$ be uniform sample distribution with $p_i = n/N$ and defined $\boldsymbol{p}_{is} = [p_1,\cdots,p_N]$ be uniform sample distribution with $p_i = ng_i/(\sum_{i=1}^N g_i)$. 
The difference between uniform sampling variance $\mathbb{G}(\boldsymbol{p}_{us})$ and importance sampling variance $\mathbb{G}(\boldsymbol{p}_{is})$ is proportional to the squared $\ell_2$ distance of the importance sampling distribution $\boldsymbol{p}_{is}$ to the uniform sampling distribution $\boldsymbol{p}_{us}$
\begin{equation*}
    \mathbb{G}(\boldsymbol{p}_{us})-\mathbb{G}(\boldsymbol{p}_{is}) = \frac{(\sum_{i=1}^N g_i)^2}{n^3 N} \|\boldsymbol{p}_{is}-\boldsymbol{p}_{us}\|_2^2
\end{equation*}
\end{restatable}

\begin{table}[t]
\caption{Summarize \emph{embedding approximation variance} $\mathbb{V}_\ell$ and \emph{stochastic gradient variance} $\mathbb{G}$ of different algorithms. $d$ is the average degree of nodes, $m$ is the size of sampled neighbors, $n_\ell$ is the size of sampled nodes in $\ell$th layer, $\beta_\ell$ denotes the upper bound of the $\ell_2$ norm of embedding vector, $\Delta \beta$ denotes the bound of the norm of the difference between the embedding and its history, $\gamma_\ell$ denote the upper bound of the $\ell_2$ norm of Laplacian matrix.}
\label{table:01_vars}
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Method}     & $\mathbb{V}_\ell$ & $\mathbb{G}$ \\ \hline\hline
\texttt{GraphSage}  & $\frac{d}{m} \beta_\ell^2 \gamma_\ell^2$ & $\frac{1}{N^2} \sum_{i=1}^N \frac{N}{n} g^2_i$ \\ \hline
\texttt{VRGNN}      & $\frac{d}{m} \Delta \beta_\ell^2 \gamma_\ell^2$ & $\frac{1}{N^2} \sum_{i=1}^N \frac{N}{n} g^2_i$ \\ \hline
\texttt{LADIES}     & $\frac{n}{n_\ell} \beta_\ell^2 \gamma_\ell^2$ & $\frac{1}{N^2} \sum_{i=1}^N \frac{N}{n} g^2_i$ \\ \hline
\texttt{GraphSaint} & $\frac{n^2}{n^2_\ell} \beta_\ell^2 \gamma_\ell^2$  & $\frac{1}{N^2} \sum_{i=1}^N \frac{N}{n} g^2_i$ \\ \hline
\texttt{MVS-GNN}    & $ d\Delta \beta_\ell^2 \gamma_\ell^2$ & $\frac{1}{N^2} \sum_{i=1}^N \frac{\sum_{j=1}^N g_j}{ng_i} g^2_i$ \\ \hline
\end{tabular}
\end{table}

\todo{problem definitions + optimization problem + SGD (LADIES + GraphSAGE)}

% In this section, we show the key challenges in training GNN using sampling based method. To see this, let us consider a GNN with two graph convolutional layers, which is general enough to illustrate the main difficulties, but is also relatively simple so that we can clearly explain the main idea and challenges.
% Define $\mathbf{L}$ as the normalized Laplacian matrix, $\mathbf{W}$ as the weight matrix, $\mathbf{X}$ as the input node feature, $\sigma(\cdot)$ as the activation function (e.g., ReLU), $\ell$ as the loss function (e.g., cross entropy), and $\boldsymbol{y}$ as the ground truth labels, the 2-layer GNN can written as
% \begin{equation*}
%     \mathbf{Z} = \sigma(\mathbf{L}^{(2)} \sigma( \mathbf{L}^{(1)} \mathbf{X} \mathbf{W}^{(1)}) \mathbf{W}^{(2)}),~\mathbf{L} = \ell(\mathbf{Z}, \boldsymbol{y})
% \end{equation*}

% Represent $\boldsymbol{\theta} = \{\mathbf{W}^{(1)}, \mathbf{W}^{(2)}\}$. In GNN, $f^{(\ell)}(\boldsymbol{\theta}) = [f_1^{(\ell)}(\boldsymbol{\theta}),\cdots, f_N^{(\ell)}(\boldsymbol{\theta})]$ with $f_i^{(\ell)}(\boldsymbol{\theta}) = \sum_{j\in \mathcal{V}} \mathbf{L}^{(\ell)}_{i,j} \mathbf{H}_j^{(\ell-1)} \mathbf{W}^{(\ell)}$. In sampling based GNN, every time a subset of nodes are sampled, only the embedding matrix and gradient based on the sampled nodes. $f_{\omega_\ell}^{(\ell)}(\boldsymbol{\theta}) = [f_1^{(\ell)}(\boldsymbol{\theta}),\cdots, f_n^{(\ell)}(\boldsymbol{\theta})]$ with $f_i^{(\ell)}(\boldsymbol{\theta}) = \sum_{j\in \mathcal{V}_\ell} \mathbf{L}^{(\ell)}_{i,j} \mathbf{H}_j^{(\ell-1)} \mathbf{W}^{(\ell)}$

% For the ease of presentation, we can represent the above GNN as a composite function of the form
% \begin{equation}
%     f(\boldsymbol{\theta}) = \sum_{i\in \mathcal{V}^{(2)}}f^{(2)}_i\left( \sum_{j\in\mathcal{V}^{(1)}} f_j^{(1)}( \boldsymbol{\theta})\right)
% \end{equation}

% When training GNN using stochastic training methods, we first sample a subset of nodes $\Tilde{\mathcal{V}}^{(1)} \subset \mathcal{V}^{(1)},~\Tilde{\mathcal{V}}^{(2)} \subset \mathcal{V}^{(2)}$, then calculate the function value $f(\boldsymbol{\theta})$ and its gradient $\nabla f(\boldsymbol{\theta})$ using the sampled nodes.:
% \begin{equation}\label{eq:sgcn_randomness}
%     f(\boldsymbol{\theta}) = \sum_{i\in \Tilde{\mathcal{V}}^{(2)}}f^{(2)}_i\left( \sum_{j\in\Tilde{\mathcal{V}}^{(1)}} f_j^{(1)}( \boldsymbol{\theta})\right),~ \Tilde{\mathbf{g}} = \left[\underset{(a)}{\sum_{i\in \Tilde{\mathcal{V}}^{(2)}}} \nabla f^{(2)}_i\left( \underset{(b)}{\sum_{j\in\Tilde{\mathcal{V}}^{(1)}}} f_j^{(1)}( \boldsymbol{\theta})\right)\right] \left( \underset{(a)}{\sum_{j\in\Tilde{\mathcal{V}}^{(1)}}} \nabla f_j^{(1)}( \boldsymbol{\theta}) \right)
% \end{equation}

% From Equation \ref{eq:sgcn_randomness}, we know there are two types of variance when using sampling based training method: (a) First-order \emph{stochastic gradient variance} introduced during backward propagation and (b) Zeroth-order \emph{function approximation variance} introduced during forward propagation. 
% Existing methods~\cite{} focus on developing a good sampling strategy to reduces \emph{function approximation variance}. However, they suffer from a high \emph{stochastic gradient variance} which slows down the convergence speed. In this paper, we propose the \texttt{MVS-GNN} that uses minimal variance sampling to reduce the First-order \emph{stochastic gradient variance} and use history activation of nodes from the previous layer to reduce the Zeroth-order \emph{function approximation variance}.
